Provable Estimation of the Number of Blocks in Block Models

Community detection is a fundamental unsupervised learning problem for unlabeled networks which has a broad range of applications. Many community detection algorithms assume that the number of clusters $r$ is known apriori. In this paper, we propose an approach based on semi-definite relaxations, which does not require prior knowledge of model parameters like many existing convex relaxation methods and recovers the number of clusters and the clustering matrix exactly under a broad parameter regime, with probability tending to one. On a variety of simulated and real data experiments, we show that the proposed method often outperforms state-of-the-art techniques for estimating the number of clusters.

==> analysis.tex <==
% Analysis
\section{Analysis}

The idea of proof is to construct a reference matrix that is feasible in the mis-specified setting, while still maintains the true structure. And we further show that asymptotically, the solution for \ref{sdp-s} concentrates to the proper reference matrix.

We define a family of feasible matrices for \ref{sdp-s}. 
\bas{
\cF_s^{ref}:=\left\{ X_s(\alpha, \beta, \gamma)\in \bR^{n\times n}: X_s=\alpha X_0+\beta E+\gamma I \right\}
}
\begin{lemma}
\end{lemma}
